Efficient pattern-based anomaly detection in a network of multivariate devices

Many organisations manage service quality and monitor a large set devices and servers where each entity is associated with telemetry or physical sensor data series. Recently, various methods have been proposed to detect behavioural anomalies, however existing approaches focus on multivariate time series and ignore communication between entities. Moreover, we aim to support end-users in not only in locating entities and sensors causing an anomaly at a certain period, but also explain this decision. We propose a scalable approach to detect anomalies using a two-step approach. First, we recover relations between entities in the network, since relations are often dynamic in nature and caused by an unknown underlying process. Next, we report anomalies based on an embedding of sequential patterns. Pattern mining is efficient and supports interpretation, i.e. patterns represent frequent occurring behaviour in time series. We extend pattern mining to filter sequential patterns based on frequency, temporal constraints and minimum description length. We collect and release two public datasets for international broadcasting and X from an Internet company. \textit{BAD} achieves an overall F1-Score of 0.78 on 9 benchmark datasets, significantly outperforming the best baseline by 3\%. Additionally, \textit{BAD} is also an order-of-magnitude faster than state-of-the-art anomaly detection methods.

==> CIKM_reviews.tex <==
%SUBMISSION: 6404
%TITLE: Pattern-Based Anomaly Detection in a Network of Multivariate Time Series
%
%-------------------------  METAREVIEW  ------------------------
%The work addresses outlier detection in a multivariate time series setting within a network. Frequent patterns in similar time series are used to define normal behavior and anomalies are found by identifying time periods without frequent patterns. While the work is interesting, it requires more refinement before publications. 
The reviewers pointed out missing citations from the literature review for the problem, improvements that could be made to the description, and the need to further analyze and discuss choices in the meta-parameters of the proposed method.

TODO: see details below

%----------------------- REVIEW 1 ---------------------
%SUBMISSION: 6404
%TITLE: Pattern-Based Anomaly Detection in a Network of Multivariate Time Series
%AUTHORS: Len Feremans, Boris Cule and Bart Goethals
%
%----------- Overall evaluation -----------
%SCORE: -1 (weak reject)
%----- TEXT:
%This paper studies the anomaly detection problem in a network and multivariate time series setting. The goal is to achieve effcient and interpretable model for anomaly detection. The authors choose a pattern-based solution to address the efficiency challenge. First, they compute the similar time series in different device to capture the interaction between devices. On top of that, they discover frequent patterns to describe normal behaviors and select the best patterns. Afterwards, they transform time series into pattern-based embeddings and search for anomalies as those time periods in which frequent patterns are missing. In general, the problem setting is novel, the proposed techniques are solid and have been evaluated better than baselines. However, 
the presentation needs to be improved. It is suggested to revise the introduction to highlight the unique network setting. It is also recommended to add a overview picture of the proposed solution.

DONE: rewrite intro, add global illustration

%----------- Strengths and reasons to accept -----------
%S1. An intersting problem in a pratical setting.
%S2. Examples are given in technical presentation.
%S3. Different datasets are evaluated.
%----------- Weaknesses and limitations -----------
W1. The motivation and problem setting are bitter to follow. Anomaly detection is a well-studied topic and apprently this paper targets a specific setting. The authors have introduced their setting in the end of the first paragraph, but it is very hard to understand the semantics of the attributes (such as those sensor names) in Table 1.

And in the introduction, there is no descriptions of what are entities and sensors.

-> DONE
%NU WEL... 

This makes it confusing to understand the significance of the proposed techniques. A feeling is that the conclusion is better-written than the introduction, which explains why they identify the similar time series in different devices and how they use the patterns to search for anomalies.

TODO: clarify intro and terminology

W2. The paper lacks an overview framework to illustrate the general workflow of their anomaly detection. This issue could be discussed together with W1. Since there is no overview picture of the solution, it is hard to follow the technical details. It is suggested to add a framework before or at the beginning of Section 3.

-> DONE

W3. There are a set of parameters in Algorithm 1. It is suggested to detail how to tune the parameters. This is an important issue for real-world deployment.

TODO: discuss

W4. Is it able to evaluate inter-device similarities using the benchmark datasets? This would be important to understand the contribution of the proposed method to the overall anamoly detection (since only benchmark datasets are used in Section 4.2).

TODO: ?

W5. In Section 2.3, there is no description of SAX. Moreover, the example in Figure 1 is not that clear. It is hard to understand the relationship between the parameters paa_win/no_bins and the result.

TODO: explain SAX, if we have space?

Minors:
- Tables 1 and 2: better to use "number of" or "# of" instead of "No". It is ambiguous.
- LIne 4 in Algorithm 1: two semicolons.

DONE. But ...

TODO: why do only If statements have semicolons (but not in Alg 2)?

%----------------------- REVIEW 2 ---------------------
%SUBMISSION: 6404
%TITLE: Pattern-Based Anomaly Detection in a Network of Multivariate Time Series
%AUTHORS: Len Feremans, Boris Cule and Bart Goethals
%
%----------- Overall evaluation -----------
%SCORE: 1 (weak accept)
%----- TEXT:
%The submission proposes a method for time series anomaly detection. Specifically, it first captures the normal the behavior of time series using frequent and cohesive sequential patterns that compress the data best using minimum description length. For computing anomalies, the authors construct a pattern-based embedding of time series of different types and use an isolation forest to make predictions. To discover similar time series based on density-based fingerprints and histograms that scale to large collections of time series. Basically, the idea is novel and the technique is sound. However, 
the related work review is far from thorough. The baselines compared are also not complete. Many SOTA deep learning-based approaches are not compared.

TODO: compare or explain why we don't compare (we do this already, we can also hope we don't get a DL fan as reviewer next time)

%----------- Strengths and reasons to accept -----------
%1)      The technology used is somehow novel.
%2)      The paper is well-written and easy to follow.
%----------- Weaknesses and limitations -----------
%Weak:
1）      the related work review is far from thorough, many deep learning based time series anomaly detection approaches are not discussed.

TODO: extend related work, if there is space

2）      The baselines compared are also not complete. Many SOTA deep learning based approaches are not compared. For example, the following ones.

A Deep Neural Network for Unsupervised Anomaly Detection and Diagnosis in Multivariate Time Series Data.
The 2019 AAAI International Conference on Artificial Intelligence (AAAI'19), 2019

Deep Autoencoding Gaussian Mixture Model for Unsupervised Anomaly Detection.
Sixth International Conference on Learning Representations (ICLR'18), 2018.

TODO: compare (or not), as above

%----------------------- REVIEW 3 ---------------------
%SUBMISSION: 6404
%TITLE: Pattern-Based Anomaly Detection in a Network of Multivariate Time Series
%AUTHORS: Len Feremans, Boris Cule and Bart Goethals
%
%----------- Overall evaluation -----------
%SCORE: -1 (weak reject)
%----- TEXT:
%This paper proposes to extract patterns from the time series data. The patterns then are applied to detect anomaly. The proposed approach can be useful for anomaly detection in IoT scenarios where data are typically time series and multiple end sensors periodically upload their readings for decision making.

1. Some technique details are not defined very clearly. For example, how to determine the granularity of the sliding windows and the fingerprint. The example shown in Figure 2 mentions the interval is 24 hours, which may be too coarse-grained.

TODO: discuss

2. The mining of edge may not be accurate. The method used by the paper is mainly based on the type of devices. What is the rationale for this? Will it be better to link the devices that are located physically close? For example, two sensors located close to each other may be affected by environmental events or attackers simultaneously.

TODO: nothing? (this is an opinion)

3. The experiments may be not too strong. It is good to see the proposed approach is tested on real-world data (S4.1). How to measure the correctness since there is no ground truth? In addition, it is unclear what insights can be revealed through these experiments.

TODO: ? (I don't really get the comment)

4. Some citations are problematic. Sometimes the unclear citing makes hard to recognize the contributions of the paper. For example (not comprehensive), line 48 needs more citation for each applications; line 86 mentions "studied extensively", but the following line has only one citation; line 190, why is [22] cited? line 204, why is [17] cited?

TODO: check

Minors:
GPU's --> GPUs

DONE

%----------- Strengths and reasons to accept -----------
%+ The paper addresses important problems. The proposed approach is potentially applicable to the emerging IoT domains.
%+ The paper is well written in general
%+ This work is motivated by and tested on real-world data
%----------- Weaknesses and limitations -----------
%- Some technical details are not well explained
%- Citations are problematic to recognize its contributions
